Astrometry and Precise Radial Velocities Yield a Complete Orbital Solution for the Nearby Eccentric Brown Dwarf LHS 1610 b

The LHS 1610 system consists of a nearby ($d=9.7$ pc) M5 dwarf hosting a candidate brown dwarf companion in a $10.6$ day, eccentric ($e \sim 0.37$) orbit. We confirm this brown dwarf designation and estimate its mass ($ 49.5_{-3.5}^{+4.3}$ $M_{\text{Jup}} $) and inclination ($ 114.5^\circ$ $_{-10.0}^{+7.4}$) by combining discovery radial velocities (RVs) from TRES and new RVs from the Habitable-zone Planet Finder with the available Gaia astrometric two-body solution. We highlight a discrepancy between the measurement of the eccentricity from the Gaia two-body solution ($e=0.52 \pm 0.03$) and the RV-only solution ($e=0.3702\pm0.0003$). We discuss possible reasons for this discrepancy, which can be further probed when the Gaia astrometric time series becomes available as part of Gaia DR4. As a nearby mid-M star hosting a massive short-period companion with a well-characterized orbit, LHS 1610 b is a promising target to look for evidence of sub-Alfv\'enic interactions and/or auroral emission at optical and radio wavelengths. LHS 1610 has a flare rate ($0.28\pm 0.07$ flares/day) on the higher-end for its rotation period ($84 \pm 8$ days), similar to other mid-M dwarf systems such as Proxima Cen and YZ Ceti that have recent radio detections compatible with star-planet interactions. While available TESS photometry is insufficient to determine an orbital phase-dependence of the flares, our complete orbital characterization of this system makes it attractive to probe star-companion interactions with additional photometric and radio observations.

==> notes.tex <==

% Winters
Only four M dwarf - brown dwarf pairs are known within 10pc.

% Sozzetti+2023
Gaia itself as a target provider for photometric and spectroscopic follow-up observations.
Holl+2022 reported on close to edge-on orbital solutions for a small sample of transiting systems identified by Kepler and TESS.
In the sample of ∼1900 candidate substellar companions presented in Gaia Collaboration et al. ( 2022a ), 49 have orbital solutions with an inclination angle in the range [89 ◦, 91 ◦], i.e. compatible with a perfectly edge-on orbit, and the median period of these solutions is ∼1.3 yr

% Sozzetti+2014
The favorable planet-star contrast ratios provided by the low intrinsic luminosity of M dwarfs allows for improved detectability thresholds of gaint planets at wide separations (5-10au) with direct imaging techniques (e.g., Bowler+2012).

% Bowler+2012
Planets Around Low Mass Stars detected substellar companions around young M dwarfs.

% Marcussen+2023
The detection of exoplanets through the astrometric reflex motion of their host stars has been predicted to revolutionize the field of exoplanetary science by increasing the total number of known exoplanetary science by increasing the total number of known exoplanets by a factor of 4 after the nominal 5 year mission of Gaia, and a factor of 14 for the extended 10 yr mission (Perryman+2014). 
The astrometric and radial velocity techniques are highly complimentary.
Gaia DR3 was published on June 13 2022.
This was the first data release where non-single-star solutions were included.
The 169,277 orbital solutions release were compiled from 34 months of Gaia observation, illustrating the potential of astrometric planet searches.
However the majority of these solutions stem from double-star systems, which produce larger astrometric signals than those from planetary systems.
In total, 1843 astrometric brown dwarf and 72 exoplanet candidates were published in DR3 \cite{arenou2022}.

% Holl+2022
\cite{holl2022} discus the exoplanet pipeline that is used for nss\_two\_body\_orbit determination.
There are 1162 sources from the exoplanet pipeline.

%\multicolumn{4}{l}{\hspace{-0.2cm} Other Stellar Parameters:}           \\
%\multicolumn{4}{l}{\hspace{-0.2cm} Spectroscopic Parameters$^a$:}           \\
%\multicolumn{4}{l}{\hspace{-0.2cm} Model-Dependent Isochrone fit Parameters:}           \\
%$T_{\mathrm{eff}}$                   &  Effective Temperature                                  & $3079 \pm 60 \unit{K}$                        & \cite{mann2015}        \\
%$M_*$                                &  Mass                                                   & $0.167_{-0.015}^{+0.014} \unit{M_{\odot}}$    & This Work  \\

% 0.1670+/-0.0042


% ------------------------------
%\subsection{Direct Imaging}
%Would GJ 3253 be amenable for direct imaging?
%What about phase-curve observations?
%Using the Sonora-Bobcat Models, GJ 3253b likely has an equilibrium temperature of X.
%This would induce a phase-curve amplitude of X.
%We checked for this in the TESS data. 

% Holl et al. 2022
The vast majority of least massive companions from Gaia DR3 are confined to $G<11$ \cite{holl2022}.
They estimate the level of spurious / incorrect solutions in the sample to be on the order of $\sim$5-10\%
The Gaia DR3 sample of known and new exoplanets and brown dwarfs orbiting bright FGK dwarfs with reliable astrometric orits is small \cite{holl2022}.
The Gaia harvest of exoplanets and brown dwarfs have converged on ballpark numbers of tens of thousands new detections \cite{lattanzi et al. 2000, Sozzetti et al. 2001, Perryman et al. 2014, Holl et al. 2022}.
These studies are provided for the end-of-mission figures, and can't be directly compared with the DR3 level sensitivity.

% Arenou et al. 2022
Multiplicity studies of ultracool dwarfs at separations $<1$au have for long been hampered by the relative faintness of those objects.
The separation and mass (or magnitude)-ratio distribution of known UCD binaries therefore carries a significant observational bias, which is also affecting the estimated UCD binary fraction of 10-30\% (e.g., Burgasser et al. 2007).
Gaia is filling in the period range of 0.5-5years in the eccentricity distribution (see e.g., Dupuy \& Liu 2017) which so far has been sparsely populated due to the resolution-limit of direct-imaging instruments.
A very large fraction of low-mass companions in Gaia are not low-mass companions, but rather binaries with a mass ratio similar to their flux ratio.
% Example astrometric orbit: https://www.cosmos.esa.int/web/gaia/iow_20220131
It is an apetizer on what we will learn from future Gaia releases.
One of the big takeaways from the paper is that the eccentricity from Gaia two body solutions sometimes don't agree.

\cite{arenou2022} have a first look at the UCD orbits in Gaia DR3.
See plots of Gaia Ucltra-Cool Dwarf Sample (GUCD \cite{smart2019}.
All such systems in GUCD in the two-boody-robit talbes have solution type OrbitalTargetedSearch.

% Sozzetti+2014
They predicted the detection of $\sim$100 giant planets detected with Gaia astrometry around M dwarfs within 30pc.
This number could be as large as $\sim$2,600 detections, and 500 accurate orbit determinations within 100pc.
10 of those could be transiting.
There are substantial synergies between astrometry and other characterization techniques.
They assumed an occurrence rate of 3-4\% of giant planets orbiting within 3au of low-mass stars. 
This large sample will enable careful estimation of occurrence rates.


% -----------------------------------
% -----------------------------------
% -----------------------------------
% Thoughts for intro from Gummi
% -----------------------------------
% -----------------------------------
% -----------------------------------

% {1} - Gaia in general
The \textit{Gaia} mission is revolutionizing the field of astrophysics already yielding insights into planets, brown dwarfs, and binaries. The detection yield of substellar objects from Gaia---including both exoplanets and brown dwarfs---has been estimated to be at the level of tens of thousands \cite{lattanzi2000,sozzetti2001,perryman2014,holl2022}. A number of new detections have been made leveraging proper motion differences between Hipparcos and Gaia allowing confirmation observations through direct imaging and/or radial velocities to be performed to gain insights into brown dwarfs \citep[e.g.,]{brandt2021,li2023} and giant planets \cite{currie2023}. Characterizing the substellar companions and the difference between brown dwarfs, and giant planets can help yield insights into how these systems form and evolve, but previous studies have highlight evidence for different formation mechanisms \citep{chabrier2014}, e.g., through their different eccentricity distributions \cite{bowler2020}.

% {2} - Two body solutions
As part of the Gaia DR3 release, 169,277 Gaia two-body solutions were published assuming a single Keplerian model derived from the first 34 months of Gaia observations \cite{Halbwachs2022}. These two-body solutions provide constraints on all orbital elements, including the orbital period, eccentricity, inclination, and mass of the companion, and correlation matrices between them assuming a dark companion. Most of these solutions are double-star systems, with around 1,162 that are likely to be substellar objects analyzed with a dedicated 'exoplanet' pipeline \cite{holl2022}. Recent work by \cite{Winn2022} provided an analysis of planets with Gaia two-body solutions, providing a framework to analyze the two-body solutions along with available radial velocity data, which in some cases highlights good agreement between the Gaia solutions, and sometimes inconsistencies. Further, follow-up observations by \cite{marcussen2023} further highlight the importance of ground-based observations to confirm and/or rule out false positive scenarios, such as double-lined systems.

%It is essential to follow-up those systems to characterize those further, and rule out false positive scenarios.
%  obtained spectra of 6 potential exoplanets detected with Gaia astrometry, demonstrating that a fraction is due to false positives.

% {3} - M dwarfs
Among different stars, nearby M dwarfs are particularly suitable for detecting substellar companions with Gaia, as they maximize the likelihood of high-precision orbit and mass determination \cite{sozzetti2014}. Around M dwarfs, \cite{sozzetti2014} predicted the detection of $\sim$100 giant planets at orbits within $3 \unit{au}$ around M dwarfs within $30 \unit{pc}$, and $\sim$$2,000$ within 100pc. Such a large sample can place tight constraints on the occurrence rates of substellar companions around M dwarfs, which still remains poorly constrained. Detecting giant planets around M dwarfs is particularly valuable, as forming such systems remains an outstanding question, given the inventory of material to form such systems is low.
% Gaia Ultra-Cool Catalog.

% {4} - We characterize GJ 3253
In this paper, we perform a detailed characterization of the GJ 3253 system, the most nearby M dwarf with a Gaia two-body solution. This system was originally detected before any Gaia two-body solutions were available by \cite{Winters2018} to be a mid M dwarf system that hosts a likely brown dwarf in a $P=10.6$day eccentric orbit with a minimum mass of $m\sin i = 44.8 \pm 3.2 M_J$ obtained with radial velocities from the TRES spectrograph. After the release of the Gaia two-body solutions, the system was highlighted in \cite{arenou2022} as the most nearby M dwarf system with a Gaia two-body solution. To characterize the system, we obtained additional precise radial velocities with the Habitable-zone Planet Finder (HPF), a near-infrared spectrograph \cite{mahadevan2012,mahadevan2014} on the 10m Hobby-Eberly Telescope. We perform a joint characterization of the available RVs, as well as the Gaia two-body solution, which allows us to constrain the orbital inclination of the companion, and thereby constrain its mass. We obtain a mass of \resm, confirming the brown dwarf nature of the companion. We place the system in context with other brown dwarf systems in Section \ref{sec:discussion}. We use available TESS data to demonstrate it has a surprisingly high flare rate. We speculate this could be due to possible interactions with its companion, although additional investigations are needed to confirm or rule out that scenario.

% Given its close proximity to Earth, and the large size of the companion around a mid M dwarf, GJ 3253 could be a promising target for star-planet interactions at radio wavelengths. 

%% ------------------------------------
%% ------------------------------------
%% ------------------------------------

\cite{holl2022} showed that Gaia's astrometric precision should allow for the detection of unseen companions down to Jupiter masses, allowing the efficient detection of large numbers of brown dwarfs.
Brown dwarfs act as a link between planets and low-mass stars, allowing insights into if they form more like high mass planets \cite{}, or through cloud fragmentation similar to low-mass stars.

TESS has discovered a number of brown dwarfs. Their masses and radii allow for constraiing BD evolutionary models \cite[e.g.,][]{chabrier2000,burrows2001,baraffe2003,marley2021}. % burrows?
There are about 30 known transiting BDs, of which M dwarfs host 9 of them.
Currently , there are eight transiting M dwarf-brown dwarf systems.
The inspiral timescale is a strong function of stellar radius, where brown dwarfs orbiting M dwarfs have larger inspiral timescales than earlier type stars.

There is a different formation mechanisms between low-and high-mass brown dwarfs 
Where high mass brown dwarfs ($>43 M_J$) are believed to form through molecular cloud fragmentation, similar to a binary stellar companion, while low-mass brown dwarfs form through gravitational instabilities in the protoplanetary disk.

% Should we have any notes on radio emission in brown dwarfs?
% Some of these could be transiting \citep[e.g.,][]{sozzetti2023}.

%It is essential to follow-up those systems to characterize those further, and rule out false positive scenarios.
%  obtained spectra of 6 potential exoplanets detected with Gaia astrometry, demonstrating that a fraction is due to false positives.


%
% 
% We use literature RVs from TRES as well as precise near-infrared radial velocities obtained with the Habitable-zone Planet Finder Spectrograph along with the Gaia two body solution to jointly characterize the RVs and astrometry for the nearby (d=9.9pc) GJ 3253 system.
% The GJ 3253 system is a nearby star with a known $m \sin i = X M_J$ brown dwarf in a $P=10.6 \unit{day}$ orbit.
% We obtain an orbital inclination of $i=X^\circ$, yielding a true mass of \resm.
% There is a discrepancy between the eccentricity of GJ 3253 from the Gaia two-body solution (e=0.5) and that from the RVs (e=0.36).
% We speculate that this could be due to X.
% Despite having a slow rotation period for a mid M dwarf, GJ 3253 shows a high flare rate of $0.2 \unit{day^{-1}}$, which could be driven by interactions with the companion, although additional observations are needed to confirm such signatures.
% Given the close-in GJ 3253 is sub-alfvenic, and would be capable of sub-alfvenic with its host star.


TOI-2119 is the most eccentric high-mass brown dwarf with a period of $<10 \unit{days}$.


% 
%In the pursuit of finding a habitable planet, we need to understand the physical mechanisms dictating the formation of substellar mass objects (i.e., brown dwarfs and planets). We question the impact of astrophysical features like stellar type or stellar mass on the resulting qualities of the companion, like its mass, radius, or orbital period. For the similar problem of stellar formation, we combined physics with observation, namely the HR-diagram, to build and test well refined relationships for age, mass, and luminosity. We can apply a similar approach for substellar mass objects by amassing observations and well derived parameters from them. 

% 
%M dwarfs are the most common stellar type in the solar neighborhood and throughout the Galaxy \citep{Latham1989}, meaning, naively, the majority of substellar mass objects we find are likely to be orbiting M dwarfs. However, gas giant planets are less common around low mass stellar hosts than they are around the more massive F and G type stars \citep{Endl2006}. This has been attributed to low mass stars having lower protoplanetary disk masses which makes it more difficult to form these larger planets (e.g., \citep{Miguel2020}). Despite these lower disk masses, gas giants planets orbiting low mass M dwarfs have been detected at long orbital periods, primarily with the RV technique. Exemplary systems are GJ 676 A b \citep{Forveille2011}, a planet with a minimum mass (m sin $i$) of 5.8 M$_{\rm{Jup}}$ and an orbital period of 1051 days orbiting an M0 star, and GJ 3512 b \citep{Morales2019}, a m sin $i$ = 0.46 M$_{\rm Jup}$ planet in a 203 day orbit around an M4 star. Of the two theories of planet formation, core-accretion struggles to account for these large mass planets, so, gravitational instability is the more favored mechanism, making the formation of these planets similar to the process of brown dwarf and stellar formation \citep{Morales2019}.

%
%As a result of the tension between formation theories for these planets, substellar mass objects orbiting M dwarfs are an excellent test bed for validation. Knowing the true mass of these objects is critical for us to determine and asses the correct theory for their formation. A drawback of the RV technique is that it only measures the minimum mass of the object, m sin $i$, because the inclination, $i$, is unknown. With only a minimum mass measurement, the true mass could be in the brown dwarf or even low-mass star regime if inclinations are close to face-on. RV surveys are also known to detect candidate objects that later turn out to be face-on binary systems (e.g., \citet{Latham1989, Wright2013}).

% 
% Recently, as part of the large Gaia Data Release 3 (DR3) in June 2022, the Gaia team released a list of 73 candidate astrometric planets, which are systems that have astrometric two-body solutions where the single dark companion mass is in the planetary mass regime. Although the Gaia astrometric time series have not been released yet, the results from fits assuming a single dark companion are provided, which include the Thiele-Innes orbital coefficients (A, B, F, G), the eccentricity ($e$), orbital period ($P$), periastron time ($t_p$), along with the covariance matrix between the parameters. These parameters can be mapped to more traditional “Campbell orbital elements”: $P$, $e$, $t_p$, argument of periastron $\omega$, angle of the ascending node $\Omega$, and the inclination $i$. Recent work by \citet{Winn2022} has shown that the covariance matrix between these astrometric parameters can be jointly sampled with RV data. This allows us to solve for the inclination, breaking the m sin $i$ degeneracy and offering the possibility to estimate true masses. 

% 
%We jointly fit the Gaia astrometric two-body solution for the system GJ 3253 with archival RVs from TRES \citep{Winters2018} and additional RVs taken with the Habitable Zone Planet Finder (HPF). We determine a true mass for GJ 3253 B of $50.91\pm0.90$ M$_{\rm Jup}$, making it a brown dwarf orbiting an M4 star.
% \cite{Winters2018} studied the GJ 3253 system using radial velocities with TRES, highlighting a companion with a minimum mass of $m\sin i = 44.8 \pm 3.2 M_J$, where the orbital inclination was unknown.

% {} - This paper is structured as follows
%This paper is structured as follows. We discuss the stellar parameters of the GJ 3253 system in Section \ref{sec:stellarparam}. We discuss the observations studied in this work in Section \ref{sec:observations}. We discuss the methods we employed for the fitting the RVs and available astrometric information in Section \ref{sec:methods}, and we show the results from these in Section \ref{sec:analysis}. We place GJ 3253 B in context of other brown dwarfs in Section \ref{sec:discussion}, and conclude in Section \ref{sec:summary}.

% The brown dwarf desert: a paucity of brown dwarf companions relative to planets at 3au around main sequence FGKM stars
% The occurrence rate of BDs is $0.7 \pm 0.2\%$ from 1000 CPS targets \citep{vogt2002,patel2007}, agreeing with measurements from McDonald Planet Search of $0.8\pm0.6\%$ from a search of 250 stars \citep{wittenmyer2009}.

% priors
\begin{comment}
\begin{deluxetable*}{llllll}
\tablecaption{Priors \label{tab:priors}}
\tabletypesize{\scriptsize}
\tablehead{\colhead{Parameter}  &  \colhead{RV-only fit}   & \colhead{RV-only Prior Type}  & \colhead{Joint Fit} & \colhead{Joint Fit Prior Type}  }
\startdata
M$_*$ ($M_{\odot}$$) & - & - & 0.1671 \pm 0.0041 & Normal     \\
m$_2$ ($M_{\rm Jup}$) & - & - & [40.0,60.0] & Uniform     \\
cosi  & - & - & [-1.0,0.0] & Uniform     \\
K (m/s) & [100000.,200000.] & Uniform & - &      \\
e & [0.0,0.9] & Uniform & [0.0,0.9] & Uniform     \\
$\omega$ (degs) & [0.0,360.0] & Uniform & [0.0,360.0] & Uniform      \\
$\Omega$ (degs) & - & - & [-180.0,180.0] & Uniform      \\
t$_{peri}$ (days) & [-6.0,6.0] & Uniform & [-6.0,6.0] & Uniform      \\
P (days) & [10.0,11.0] & Uniform & [10.3,10.7] & Uniform      \\
$\varpi$ (mas) & - & - & 103.879 \pm 0.023 & Normal      \\
$\gamma_{\text{TRES}}$ (m/s) & [-2000.0,2000.0] & Uniform & [-2000.0,2000.0] & Uniform      \\
$\gamma_{\text{HPF}}$ (m/s) & [-17000.0,17000.0] & Uniform & [-17000.0,17000.0] & Uniform   \\
$\varepsilon$ & 0 & Fixed & 0 & Fixed \\
\enddata
\tablenotetext{}{Probably need to explicitly mention $\varepsilon$ and $\sigma_0$ in the methods section.}
\end{deluxetable*}
\end{comment}


% ----------------------
%\subsection{Doppler/RV-only fit}
%The second column of Table \ref{tab:results} summarizes the results from the Doppler only fit. We compare our results to \cite{Winters2018} which discovered the secondary using only the TRES RVs. All of our values fall within the error bars of the \cite{Winters2018} results. The additional HPF RVs allow us to significantly improve precision on multiple parameters. In particular we are able to improve the uncertainty on the orbital period by a factor of 140. The semiamplitude error precision is improved by a factor of 2. Eccentricity error precision is improved by a factor of 3. Precision on the error of $\omega$ is improved by less than a factor of 2. Finally, the precision on the periastron time error is improved by a factor of 3.5.

% ----------------------
%\subsection{Astrometry}
%The values for the astrometric data reported by Gaia DR3 are shown in the third column of Table \ref{tab:results}. We can compare the values for eccentricity ($e$), argument of periastron ($\omega$), time of periastron ($t_p$), and period ($P$) directly between the RV-only and Gaia fits. We find that the RVs constrain the eccentricity to a distinctly smaller value than Gaia. Eccentricities from Gaia can often be incorrect, as they are dependent on the number of data points and the inclination, so for this close to edge on system, it can be hard to fit the eccentricity correctly (this is the impression I've gotten from talking with well-versed Gaia users. I have no citation so may be a sketchy claim to make).
%The values for $\omega$ differ by roughly 180 degrees. There is a modulo $\pi$ degeneracy in this angle for astrometric orbits that can be broken by RV information. The RVs constrain the period much more precisely and is more trustworthy than Gaia as we have a long baseline and likely more RV than astrometric points (this might not be true need to check the number of astrometric points). The time of periastron ($t_p$) is better constrained by the RVs as a consequence of the more precise fits of the argument of periastron and period. An important note is that the inclination for Gaia sets the direction of the orbit. Since the inclination falls in the realm [$\frac{\pi}{2}$,$\pi$], the orbit must be clockwise. As a result, we can fix our prior in the joint fit for the parameter cos$i$ to be between -1.0 and 0.0 since this orbit must be clockwise and the inclination can only hold values in this range as a result. 

% ----------------------
%\subsection{Joint Doppler+Astrometry Fit}
% Also when we show the mass constraints I would like to have a table with 3 different mass determinations like Benedict 2016, Mann 2018, and Giovinazzi 2022
%The results of the joint fit are shown in the fourth column of Table \ref{tab:results} and the fit to the RV points on the top of Figure \ref{fig:jointfit}. We see residuals of the RVs in line with their median errorbars. We also show the Z-score for the Thiele-Innes coefficients A, B, F, and G, as well as the eccentricity, period, and time of periastron in the bottom panel of Figure \ref{fig:jointfit}. The mass of our primary is computed using the \cite{mann2019} relationship, which determines the mass based on the 2MASS K magnitude. With the precision of our other measurements, this is the primary driver of the error on the mass of the secondary. We find the true mass of the brown dwarf to be $50.91 \pm 0.9$ Jupiter masses. The inclination of this system comes out to $117.19^{+0.88}_{-0.91}$ degrees, which is 24 degrees higher than the value expected by Gaia. The eccentricity fits closely to the RV only solution. The solution for $\omega$ is constrained by the RVs, and is consistent with the Gaia solutions by a 180 degree rotation. $\Omega$ comes out as a negative number to satisfy the fit due to the RV constraining $\omega$ to a value unexpected by the Gaia solution. If we followed the steps outlined in Appendix A of \cite{Halbwachs2022} and added $\pi$ to both $\omega$ and $\Omega$ (since $\Omega$ is negative) then we would produce roughly the same angles that the Gaia only solution produces. We find that the Z-scores are the same if we use $\Omega$ and $\omega$ in either the format shown in the Gaia Two-Body solution column or the format in the Joint Fit column of Table \ref{tab:results}. While that is true, the RVs constrain $\omega$ to the 89.31 degrees value so we consider the Joint Fit column format to be the correct values to use for $\Omega$ and $\omega$. The time of periastron value is dominated by the RVs. The period is extremely well constrained, dominated by the RV solution. 

% where for the mass of the primary star we used the M-K relationship from \cite{mann2019}. We estimated primary masses using the M-K relationship which is based on the distance and 2MASS K magnitude. We then used the two-body-solution constraints on the orbital parameters to estimate the RV semi-amplitude and then the mass of the secondary. 


%Of note, they list a mass of $0.052 \pm 0.004 M_\odot$ ($54.5 \pm 4.19 M_{\text{Jup}}$) for the secondary when assuming a primary mass of $0.17 \pm 0.02 M_\odot$. They find a period, $P = 10.5885 \pm 0.0013$ days and an eccentricity, $e = 0.524 \pm 0.027$.

% In the \cite{Reyle2021} database, there are $\sim$100 brown dwarfs known within 10 parsecs of the Sun. Of these, 8 have publshed dynamical masses. The measured masses of these targets are: Luhman 16 A = $34.2^{+1.1}_{-1.3}$ $M_{\rm Jup}$ and Luhman 16 B = $27.9^{+1.0}_{-1.1}$ $M_{\rm Jup}$ \citep{Garcia2017}, $\varepsilon$ Indi B = $75.0\pm 0.8$ $M_{\rm Jup}$ and $\varepsilon$ Indi C = $70.1\pm 0.7$ $M_{\rm Jup}$ \citep{Dieterich2018}, GJ 229 B = $71.4 \pm 0.6$ $M_{\rm Jup}$ \citep{brandt2021}, Scholz's Star B = $66  \pm 4$ $M_{\rm Jup}$ \citep{Dupuy2019}, GJ 569 Ba = $80^{+9}_{-8}$ $M_{\rm Jup}$ and GJ 569 Bb = $58^{+7}_{-9}$ $M_{\rm Jup}$ \citep{Dupuy2017}. 

% We find that within 10 parsecs, GJ 3253 B is the fourth most precisely measured dynamical mass of a brown dwarf. More precise measurements are known for $\varepsilon$ Indi B and C as well as for GJ 229 B. GJ 229 B and $\varepsilon$ Indi C are measured to better than 1$\%$. 

% An analysis of the Kepler and Corot samples of short-period transiting brown dwarfs revealed that they are rare with an occurrence rate of 0.2-0.3\% around sun-like stars. There are 48 transiting brown dwarfs, 9 of which have M dwarf host stars. From a statistical analysis of the brown dwarf population, \cite{Ma2014} postulated the brown dwarf sample is comprised of two populations: i) a low-mass group with $M<42.5 M_J$ with an eccentricity distribution comparable to gas giants, and (ii) high-mass group with an eccentricity distribution comparable to binary stars. GJ 3253 B falls in the high mass regime and has a relatively high eccentricity given its period and mass.  Figures 2 and 3 in their work show a depletion of brown dwarfs with periods less than 100 days and masses between $40$-$60$ Jupiter masses. GJ 3253 B peculiarly sits in the center of this sparsely populated region.

% We expect contribution from ellipsoidal variations to be negligible.
% Marley et al. 1999 provide an estimate of the geometric albedo of $A_g \sim 0.1$ for a massive brown dwarf oribiting an early M dwarf.

% The orbit of GJ 3253 B is not evolving due to tides and should remain unperturbed for the main-sequence lifetime of GJ 3253.
% The circularization timescale is only comparable to the system age for a few million years and the eccentricity of the system has probably not changed significantly due to tides.
% specifically the evolution tables for solar metallicity and C/O ratio of 1,
% The value could dramatically change if spin rates for brown dwarfs are much higher or lower than for Jupiter-like objects and if the tidal dissipation factor is incorrect.

% The data points are drawn from a compilation of objects with masses between 13 and 80 Jupiter masses in the NASA Exoplanet Archive, the Exoplanet.EU catalog, and BD-M dwarf binaries with dynamical masses in the literature.
% An upper bound was placed on the host mass at 0.6 solar masses to encompass BD-M dwarf binaries. 
% Objects shown have mass measurements with precision greater than 3$\sigma$.

% Gaia will significantly increase the number of giant planets and brown dwarfs around nearby stars, enabling us to further characterize the eccentricity distributions of substellar objects. 
% Building out this dataset will help us further our understanding of the formation of substellar mass objects.
We limited the labeled points to those with stellar host effective temperatures between 2000-4000 K to better represent M-dwarfs.
We only include points if they have associated errors for the period and eccentricity.
We only include points that have a companion mass error measurement better than 33\% and a stellar mass measurement below 0.6 $M_{\odot}$. The faint points are targets from the Gaia two-body-solutions table. Eccentricity, period, and distance of these points come from the Gaia fits, while we estimate masses based on the K-magnitude of the host star and the distance \citep{mann2019}.

% to query the sector-by-sector PDCSAP flux, clear it of \texttt{nan} values and use the \texttt{lightkurve} function, flatten, to smooth the data over 400 minute windows. 
% We compute the standard deviation of this flattened lightcurve, then reload the data and follow the same steps, but instead of flattening, we use the normalize function. 
% The normalized lightcurves are sent through \texttt{stella} with a probability threshold set at 0.6. 
% We remove false positives by removing flares with fractional amplitudes less than 3 times the standard deviation we calculated prior, or rise+fall times less than 4 minutes (two TESS cadences). 
% After this step, sectors are reviewed by eye to add or remove any flares that were misidentified. 
%The flare rate is then computed as the total number of flares divided by the observing baseline. 
%We compute flare rate uncertainties using 1-$\sigma$, two sided Poisson confidence intervals. 
%Using these steps we compute a flare rate of $0.28 \pm 0.07$ flares per day.
% Our methodology to detect and identify the flares is discussed in Section \ref{subsec:TESS}. 
Across all of the sectors we detected 17 flares, 4 in Sector 42, 6 in Sector 43, and 7 in Sector 44. 
With the baseline of 61.6 days this results in a flare rate of $0.28 \pm 0.07$ flares per day. 

% The flares are visualized in Figure  uses our fits for the orbital elements and the package \texttt{rebound} \citep{rebound,reboundias15} to show the orbits of the host star and companion in the center of mass frame, from the observers perspective. 
% We compute the phase of each flare by phase-folding the TESS sectors over the period and centering at the periastron time, shown in the middle panel. 
%We show the position of the host and the companion for each flare. 
%The points are color-coded by the log of the energy of the flare. 
%Corresponding positions between the host and companion will have the same color and can be determined by taking a point on one of the ellipses and drawing a line straight through the center of mass to the other ellipse. 
%This is demonstrated by the dotted line connecting the two squares which represent the positions of the star and companion at periastron. 
%The red line is the rotation axis, normal to the orbital plane. 
%Note that this orbit is inclined 117.19 degrees and the objects orbit clockwise.
%\cite{pass2023} studied activity of nearby M stars.
% We use the model of \cite{lanza2009} and \cite{turnpenney2018} to estimate.

% Several studies of individual systems with close-in and eccentric hot Jupiters report excess flaring in phase with the planet or close to periastron \cite{shkolnik2005} although a number of similar systems do not show such excesses (CITE). 
% Multiple physical models of SPI-induced flaring exist, e.g., \cite{saur2013} and \cite{lanza2018}.
% Flares can be triggered intrinsically by the star in isolation, and also through star-companion interactions \cite{saur2013,lanza2018}, where the latter case the flare is induced by the re-connection of stellar and companion magnetic field lines.
% For that to occur the companion has to orbit the star in a close orbit, within the Alfven radius.
%It is unclear if GJ 3253 is observed equator on as we do not have a constraint on the stellar inclination.
% Absence of flaring SPI signals are also informative, which would favor models with strong stellar winds that produce small Alfven zone, and steady energy transfer channels between the companion and the star instead of eruptive and flaring channels.
% A variation of flaring rate with stellar rotational phase is expected as extremely active regions move in and out of view.
% There are observational biases: flares could be too low energy to detect in TESS. 
% They could be too infrequent to build up a high enough SNR of detection. 
% The flare region could be at high latitudes and be geometrically foreshortened decreasing feasibility of detection.
% where a preference for flaring at certain orbital phases---such as close to periastron---could  
% A statistically significant orbital phase dependence of flaring is the closest we can get to detecting evidence of flares.

% This flare rate is high compared to other radio emitting M stars from \cite{pope2021}.
% Comparing this value to flare rates of other radio emitting M-dwarfs in Table 1 of \cite{pope2021}, it is surprisingly high for the rotation period. 
%Stars with similar flare rates, like DO Cep and LP 259-39, have rotation periods of 0.41 and 1.7 days respectively. GJ 625 has a rotation period comparable to GJ 3253, but a flare rate upper limit of 0.036. 
% Additional observations with sensitive radio observatories, such as LOFAR could yield further insights into this possibility.

%This flare rate is a flare rate above a certain energy.
%Several of these host planets and have radio detections potentially induced by star-companion interactions. Specifically, Proxima Centauri has comparable X-ray activity to GJ 3253 as mentioned in Section \ref{subsec:xray} and a comparable optical flare rate in Figure \ref{fig:flares}. 
%Considering the radio detections from Proxima Cen in \cite{Perez-Torres2021}, GJ 3253 becomes a compelling candidate for radio investigation for star-companion interactions.
%Flare energies are computed as outlined in \cite{Medina2020} and as summarized here: we compute the luminosity of the star in the TESS bandpass using the TESS magnitude of the star, the zero-point magnitude flux of TESS ($4.03 \times 10^{-6}$ ergs cm$^{2}$ s$^{-1}$), and the distance determined using the Gaia parallax from Early Data Release 3. 
%We multiply this luminosity by the equivalent duration of each flare as determined by \texttt{stella}, which gives us the energy of a given flare. 
%They identify flares in 2-minute cadence TESS sectors by correcting for variability with a Gaussian process (GP) in the package \texttt{exoplanet} \citep{Foreman-Mackey2017,foreman_mackeyexoplanet}. 
%They subtract the GP model from the data and denote flares as signals with at least 3 consecutive 3-$\sigma$ outliers. By calculating energies as described above, they consider true flares to have energies greater than log(E/ergs) >= 31.5 in the TESS bandpass. 
%They implement a completeness correction on their data to account for the distance to the stars and fit a flare frequency distribution for their sample to determine their final flare rates. 

% ----------------------
% ----------------------
% ---------------------- X-ray notes
% ----------------------
% ----------------------
%\subsubsection{X-ray Detections}\label{subsec:xray}
%Stellar magnetic fields induce coronal temperatures that result in X-ray emission. 
%In solar-like stars, those with radiative cores and convective envelopes, shearing due to differential rotation at the boundary of these regions, called the tachocline, is thought to be the dynamo of the stellar magnetic field \citep{Parker1955,Babcock1963,Spiegel1992}. 
%However, using the Chandra X-ray Observatory \citep{ChandraXRT}, \cite{Wright2016} showed that GJ 3253, among other fully convective M-dwarfs like Proxima Centauri, is consistent with the rotation-activity trend in the X-ray unsaturated regime that is derived from solar-like stars. 
%This could mean that the dynamo of solar-like stars is more similar to fully convective stars than previously thought \citep{Irving2023} or M-dwarfs have a different mechanism \citep{Durney1993} that results in similar levels of X-ray emission. 
%It is also worth considering if star-companion interactions are inducing activity due to interactions between the objects' magnetic fields.

%\cite{Wright2016} determine GJ 3253 to have a fractional X-ray luminosity, 
%$\log(\frac{L_{\text{X}}}{L_{\text{bol}}}) = -4.3$.
%Using our SED computed bolometric luminosity of $0.00318 \unit{L_{\odot}}$, we compute GJ 3253 to have a $\log(L_{\text{X}}$) of 26.8. 
%Using the radius from our SED fit, we find the X-ray surface flux to be $\log(F_{\text{X,SURF}}) = 5.4$. 
%This places GJ 3253 non-uniquely into the sample of \cite{Caramazza2023}, specifically their Figures 2 and 3. 
%GJ 3253 does not exhibit an abnormal level of X-ray emission, leading us to conclude that it should be as magnetically active as other stars near it in the rotation-activity trend. 
%To compare activity we can use the similar star Proxima Centauri (M5.5), which has a fractional X-ray uncertainty, $\log(\frac{L_{\text{X}}}{L_{\text{bol}}}) = -4.3$ \citep{Wright2016}, 
%$\log(L_{\text{X}}) = 27.2$ \citep{Schmitt2004} and $\log(F_{\text{X,SURF}}) = 5.9$ when assuming a radius of $0.168 R_{\odot}$ from TESS.
% ----------------------
% ----------------------
% ----------------------
% ----------------------
% ----------------------

% The bottom panel of Figure \ref{fig:mass_precision} shows the brown dwarf orbital eccentricity as a function of orbital period, where the points are colored by the host star mass. We see that with an eccentricity of $e=0.37$ GJ 3253 B has an eccentricity in the upper envelope for objects within $<10,000$ day orbits, and it is only GJ 229 B---which has a substantially higher orbital period of $P\sim10^5 \unit{days}$---that has a higher eccentricity. There is an observed circularization period trend of M-dwarf binaries at $\sim$$10$ days \citep{Udry2000, Mayor2001} as well as for Sun-like binaries at $\sim$$10$-$12$ days \citep{Duquennoy1991, Meibom2005, Raghavan2010}. The dashed line in Figure \ref{fig:mass_precision}B shows the maximum eccentricity where the object would be unaffected by tides if we set the cutoff period to 10 days. GJ 3253 B is inconsistent with the 10 day circularization period, and is more consistent with a circularization period less than $\sim$$8$ days like the $\sim$$3-5$ day circularization period suggested for giant exoplanets \citep{Halbwachs2005,Pont2011,Bonomo2017}.

% However, GJ 3253 B is observed to occupy the Brown Dwarf 'depletion gap' between $35 - 55 M_J$ where short-period ($P<100 \unit{days}$) brown dwarfs are observed to be depleted \citep{ma2014}. 
% Further, with an eccentricity of $e=0.37$, GJ 3253 B is compatible with the upper limit of eccentricities produced by scattering simulations of \cite{Ford2008}. 
%of brown dwarfs from 
%fits with the upper envelope of possible eccentricites 
%but with a period of 10.6days and eccentricity of $e=0.37$, GJ 3253 B occupies a region devoid of other systems. 
%For the eccentricity-mass relationship, GJ 3253 B is consistent with the high-mass regime but would also fit with the trends of \cite{Ford2008}, suggesting consistency with the low-mass regime. 
%Due to the similarities to both regimes, it is difficult to confidently say which distribution, and thus which formation pathway, GJ 3253 B comes from.
% but it resides in the depleted region observed in their mass-period relationship
% In the eccentricity-period distributions, GJ 3253 B is more consistent with the low-mass points.

% Recently \cite{trigilio2023} and \cite{pineda2023} detected radio signatures at repeating phases in the YZ Ceti system.

% With respect to searching for signatures of modulation in stellar activity indicators similar to reported by \cite{shkolnik2005}, we see no evidence of emission in any of the 6 HPF visits in the Ca II IRT activity indicators. However, due to the 
% Previous work by \cite{ilin2022} looked at evidence of phase-dependent flaring in AU Mic, a nearby young and active M star hosting two transiting planets, concluding that although AU Mic shows the largest number of flares detected among all exoplanet hosts found by Kepler and TESS, most of the flares are likely manifestations of intrinsic stellar activity rather than due to star-planet interactions.

% Additional observations, including at radio wavelengths, which are particularly sensitive to detecting sub-alfvenic interactions would be beneficial to study if any further evidence could be found for radio detections.

Corresponding positions of the star and brown dwarf when flares occur. Points are color-coded by the log of the energy of the flare. Corresponding positions between host and companion have the same color and are determined by drawing a line straight through the center of mass from one ellipse to the other, demonstrated by the dotted line connecting the two squares representing the periastron positions of the star and companion.   will be included with the manuscript
% To estimate flare rates of GJ 3253, we analyzed the 2 minute cadence presearch data conditioning single-aperture photometry (PDCSAP) light curves using the \texttt{stella} code \citep{feinstein2020stella,feinstein2020}, which ensembles a set of trained Convolutional Neural Networks (CNN) to identify flares. Following the methods of \cite{pope2021} to determine a flare rate we use the package \texttt{lightkurve} to query the sector-by-sector PDCSAP flux, clear it of \texttt{nan} values and use the \texttt{lightkurve} function, flatten, to smooth the data over 400 minute windows. We compute the standard deviation of this flattened lightcurve, then reload the data and follow the same steps, but instead of flattening, we use the normalize function. The normalized lightcurves are sent through \texttt{stella} with a probability threshold set at 0.6. We remove false positives by removing flares with fractional amplitudes less than 3 times the standard deviation we calculated prior, or rise+fall times less than 4 minutes (two TESS cadences). After this step, sectors are reviewed by eye to add or remove any flares that were misidentified. The flare rate is then computed as the total number of flares divided by the observing baseline.  We compute flare rate uncertainties using 1-$\sigma$, two sided Poisson confidence intervals. Using these steps we compute a flare rate of $0.28 \pm 0.07$ flares per day.

%We quantify this by determining the number of flares expected in a region of phase space based on our flare rate and the number of orbits observed in the data. 

% For half of the orbit shown in Figure \ref{fig:flares}, we would expect $8.6 \pm 2.2$ flares over the baseline of the observations. The half of the orbit encompassing periastron would consist of the phase values between -0.25 and 0.25 in Panel D of Figure \ref{fig:flares2}. In this region we find 9 flares, while outside of this region, there are 8 flares. This is consistent with expectation and quantitatively supports that there is no preference for flaring near periastron. 

% Estimated power from star-planet interactions (top) and from direct auroral emission of the brown dwarf (bottom). \textbf{Top:} The estimated power produced via sub-Alfv\'enic interactions between GJ~3253~B and its host star as a function of orbital phase, for an age of 7~Gyr. A fraction of this energy is expected to enhance emission from the host star in the form of hotspots at the surface, and also power bright radio emission along the magnetic field line connecting the two bodies. The purple and orange lines show the power in the case where the brown dwarf is magnetised and unmagnetised, respectively. The solid line and the shaded regions show the median and the $1\sigma$ region, respectively. An orbital phase of zero corresponds to the orbit periastron. \textbf{Bottom:} Same as above, but for the stellar wind power incident on the magnetosphere of GJ~3253~B. We again assume an age of 7~Gyr for the brown dwarf. A fraction of this power is expected to drive auroral emission near its magnetic poles.

% However, such signatures may be difficult to distinguish from the quiescent emission of the star \citep{saur21}.

% However, it is unclear how practical such emission would be to disentangle from the host star.

 to enhance emission from the host star in the form of hotspots at the surface, and also power bright radio emission along the magnetic field line connecting the two bodies. For the wind-magnetospheric power, a fraction is also expected to dissipate, but instead near the magnetic poles of the brown dwarf manifesting as auroral emission. Note that auroral emission is only possible if the brown dwarf possesses an intrinsic magnetosphere

 %\title{Characterization of the close-in Eccentric Brown Dwarf Orbiting the Nearby Mid M Dwarf GJ 3253 Using Gaia and Radial Velocities}

 % Old Abstract
 Brown dwarfs are rare companions to main sequence stars. We characterize the GJ 3253 system, a nearby ($d=9.9 \unit{pc}$) M5 dwarf known to host a brown dwarf in a short period eccentric orbit with a minimum mass of $m\sin i \sim 44.8 \unit{M_J}$. A joint fit of the available Gaia two-body solution and new radial velocities (RVs) obtained with the Habitable-zone Planet Finder Spectrograph combined with literature RVs from TRES yields a precise orbital period of $10.594733 \pm {0.00002}$ days and eccentricity of $0.37004\pm 0.0003$. The astrometry allows us to constrain the orbital inclination of $117.2\pm0.9^\circ$ yielding a mass constraint of \resm, the second most precise mass constraint of brown dwarfs orbiting M stars within 25pc. We highlight a discrepancy between the eccentricity of GJ 3253 from the Gaia two-body solution ($e=0.52 \pm 0.03$) and that from the RVs ($e=0.3702\pm0.0003$), which we attribute to imperfect modeling of the Gaia astrometry. GJ 3253 B also has the second highest eccentricity for  Despite having a slow rotation period of 84.3 days for a mid M dwarf, GJ 3253 shows a high flare rate of $0.28 \pm 0.07$ flares per day in TESS photometry, which we hypothesize could be due to star-companion interactions,  although additional data will be needed to confirm or refute such interactions. Given GJ 3253's close proximity to Earth and large size of the short-period companion, we show that the GJ 3253 system is a promising target to search for signatures of star-companion interactions and direct auroral emission from the brown dwarf at radio wavelengths.
 %

 %\textbf{Assuming $\sin i$ equal to 1, the rotation period indicates a rotational velocity of 0.12 $\pm$ 0.01 km/s.}

 % \textbf{The flare rate we derived from the TESS lightcurves of LHS 1610 place it on the high end for its rotation period amongst the volume-complete sample of mid-to-late M dwarfs within 15pc from \cite{Medina2020} and \cite{Medina2022}. Within this sample, LHS 1610 is similar in spectral type, flare rate, and rotation period to Proxima Centauri and YZ Ceti, both of which have observed radio emission attributed to possible star-companion interactions. Using the available TESS data, we explored if there was any We do not demonstrate signs of star-companion interactions in the LHS 1610 system in this work, but instead evaluate the feasibility of detecting such interactions in the radio with future possible efforts.}

% \textbf{We simulated both the expected energetics 
% We demonstrate that LHS 1610 b resides in a sub-Alfvénic orbit over its variable range of orbital distances, a necessary component for star-companion interactions. We show that given even conservative estimates, the radio emission expected from the star due to these interactions is within the sensitivity range of LOFAR. Even in the absence of sub-Alfvénic interactions, we may detect auroral radio emission from the brown dwarf. The detection of either of these interactions is dependent on the orbital phase of the brown dwarf, which benefit from the full orbital solution and precise ephemeris provided in Table \ref{tab:results}.}

% \textbf{To determine the orbital elements the Gaia team fit the astrometric data with a model that also includes parallax, position, and proper motion}. 
%The Campbell elements are adopted as listed in the Gaia table.

% Our period is covariant with $t_p$ and F. Both $P$ and $t_p$ are precisely constrained by the long-baseline RVs.
% The central criterion to enable star-companion interactions is that the companion must 

The total likelihood is the log value of the priors added to the summation of the log values of the likelihood function for each RV point.

% \textbf{To check if the assumption that the secondary companion is 'dark' and contributes no light, as assumed in the Gaia two-body solutions, we estimate the flux ratio between the brown dwarf and host star in the Gaia bandpass. Using the Sonora-Bobcat spectral templates \citep{marley2021} for the brown dwarf, PHOENIX stellar spectral templates \citep{Husser2013} for the star, and accounting for the transmission curve across the Gaia bandpass, we estimate the flux ratio in the Gaia bandpass (320-1100 nm) to be negligible (less than $10^{-6}$), and we do not expect light emitted from the brown dwarf to impact the Gaia solution.}


%We perform a detailed characterization of the LHS 1610 system, a nearby ($d=9.7 \unit{pc}$) M5 dwarf known to host a brown dwarf in a short period eccentric orbit. A joint fit of the available Gaia two-body solution, the discovery radial velocities (RVs) from TRES, and new RVs obtained with the Habitable-zone Planet Finder Spectrograph, yields an orbital period of $10.594733 \pm {0.00002}$ days and eccentricity of $0.37004\pm 0.0003$. The newly constrained orbital inclination of $117.2\pm0.9^\circ$ yields a mass constraint of \resm. This gives LHS 1610 b the second most precise mass of brown dwarfs orbiting M stars within 25pc, behind only GJ 229 B. We highlight a discrepancy between the Gaia two-body solution eccentricity ($e=0.52 \pm 0.03$) and that from the RVs ($e=0.3702\pm0.0003$), which requires the astrometric time-series release (Gaia DR4) for further diagnostics. With a TESS photometry derived flare rate of $0.28\pm 0.07 \unit{flares/day}$ and a rotation period of $84 \pm 8$ days, LHS 1610 joins other mid M stars---including Proxima Centauri and YZ Ceti---as nearby mid M dwarfs with flare rates at the higher end for their long rotation periods. These stars are promising candidates for searching for sub-Alfvénic star-companion interactions. raising the question if LHS 1610 b could be driving the flares on its host via such interactions. However, we find no statistically significant orbital phase-dependence of the flares in the TESS data. We show that with a large, short-period companion around a nearby mid M star, the LHS 1610 system is a promising target to look for evidence of star-companion interactions or aural emission from the brown dwarf at radio wavelengths.



===============================
===============================
===============================

%Our B value is smaller by $\sim$10 sigma, $e$ is smaller by $\sim$5 sigma, and $P$ is larger by $\sim$5 sigma. From the covariance matrix, B has the strongest covariance with $e$ compared to the other Thiele-Innes coefficients. As such, we suspect the explanation for the strong shift in eccentricity leads to this dramatic difference for B and the inclination. Further investigations into those correlations require access to the raw Gaia astrometry, which will be available with the Gaia DR4 release. 

% \subsection{\updated{Discrepancies between Gaia and RV Results}}
% \updated{Without the actual astrometric data we are left to evaluate the results of the sampling via indirect methods. One such way is to separate equation \ref{eq:Winneq17} into the 2 principles that it is built on, Kepler's Third Law and the assumption that the photocenter is the flux-weighted mean position between the two objects. These equations are
% \begin{enumerate}
% \item \textbf{Kepler's Third Law:}
% \begin{equation}
% a = \varpi \left( (M_* + M_{BD})P^2 \right)^{1/3}
% \end{equation}
% \item \textbf{Relationship between $a_0$ and $a$}
% \begin{equation}
% a = a_0 \left( \frac{M_* + M_{BD}}{M_{BD}} \right)
% \end{equation}
% \end{enumerate}
% If we use the values from our joint sampling we find that for case 1. $a =  5.883\pm0.038$ mas and for case 2. $a = 5.881\pm0.146$ mas. This demonstrates consistency and highlights how the joint sampling determines the final values for the sampled parameters. Since we have the actual RVs and can analyze the residuals between the models, we are motivated by the joint sampling's convergence on the same values for the parameters that it shares with the RV-only fit. The joint sampling only adjusts the parameters it shares with the Gaia two-body solution based on their covariances and the indisputable information we get from the RVs.

% For completion we will highlight several different methods we may use to estimate the mass of the brown dwarf.
% These are summarized in table \ref{tab:massestimates} and are done as follows:

% \begin{enumerate}
% \item  \textbf{Mass Estimate 1:} 
% We can assume that the Gaia two-body solution value for the inclination is correct and pair this with our new msini. Using this inclination of $92.8\pm1.9^\circ$, we compute a true mass of the brown dwarf of $44.46\pm0.68$ $M_\text{Jup}$. However, due to the distinct disagreement between the RV-only and Gaia two-body solution values for the eccentricity, we are not motivated to use the Gaia two-body solution values as they are.
% \item  \textbf{Mass Estimate 2:} Using equation 15 in \citet{Winn2022}:
% \begin{equation}
% K = \frac{2\pi}{P} \frac{(a_0/\varpi) \sqrt{1-\text{cos}^2 i}}{\sqrt{1-e^2}}
% \end{equation}
% we can derive the inclination, $i$. The parallax is unambiguously determined from the Gaia astrometry independently of the two body solution. If we input $K$, $P$, and $e$ from the RV only fit, while $a_0$ and $\varpi$ come from the Gaia only solution, then we derive an inclination of $122.1\pm2.5^\circ$. Pairing this with the msini from the RVs, we determine a mass of $52.4\pm1.6$ $M_\text{Jup}$. 

% \item \textbf{Mass Estimate 3:}
% Estimate 2 doesn't account for the covariances between the Gaia only values but the joint sampling does. This is why we are  If we again follow the same steps as above to check the agreement across equation \ref{eq:Winneq17}, we find that using the joint sampled values results in 
% left hand side =
% right hand side =
% which shows agreement and motivates our trust in these values.
% \end{enumerate}

% We acknowledge the differences between the RV only fit and the Gaia only solutions. These discrepancies cannot be fully dissected until the release of Gaia DR4, but given the discussion above, we are motivated to move forward with the values from the joint sampling (final column of Table \ref{tab:results}) as our results for the orbital elements and mass of LHS 1610b.}

% To be complete, we may assume that because the $e$ and $P$ errors are underestimated, then all of the parameter errors are underestimated. Such an underestimate will lead to an underestimation of the errors on our final results for parameters which require input from the Gaia two-body solution to be constrained. In order to utilize the Gaia solution properly, given that it has a clear disagreement with the RVs, we do not fix the inflation factor to 1 and allow it to be fit. 

%The latter reduced the weight the Gaia covariance matrix plays in the joint likelihood function, anchoring the solution to the RV-derived parameters, while still yielding reasonable constraints on 
%increased the relative uncertainties in the Gaia covariance matrix, 
%where the latter inflated the Gaia covariance matrix by a scaling factor while keeping the relative covariances between the paramters.
%a likelihood function that jointly sampled the available Gaia covariance matrix along with a a likelihood function that fit the available radial 
% Gaia reports $\Omega = 162.6$ degrees and $\omega = 271.4$ degrees. Our joint \updated{sampling} produces

%\begin{abstract}
%We characterize the LHS 1610 system, a nearby ($d=9.7$ pc) M5 dwarf hosting a brown dwarf in a $10.6$ day, eccentric ($e \sim 0.37$) orbit. \updated{Radial velocities (RVs) obtained with the TRES and Habitable-zone Planet Finder spectrographs suggest a minimum mass of $44.38\pm0.67$ $M_{\text{Jup}}$. Additionally, we perform a joint \updated{sampling} of the the radial velocities and the covariance matrix from the Gaia astrometric two-body solution available for the system, resulting in an inclination of $i=114.5^\circ$ $_{-10.0}^{+7.4}$ and a true mass of $m=49.5_{-3.5}^{+4.3}$ $M_{\text{Jup}}$, confirming the brown dwarf nature of the system. We highlight a discrepancy between the astrometric Gaia two-body solution and the radial velocity solution, which results in different eccentricities of $e=0.52 \pm 0.03$ and $e=0.3702\pm0.0003$, respectively. We discuss possible reasons for this discrepancy, and we urge for further investigations of the cause for this discrepancy when the Gaia astrometric time series become available as part of Gaia Data Release 4.} With a flare rate of $0.28\pm 0.07$ flares/day from TESS photometry, and a rotation period of $84 \pm 8$ days, LHS 1610 joins other mid M stars---including Proxima Centauri and YZ Ceti---as nearby mid M dwarfs with flare rates on the higher end for their long rotation periods. These stars are promising candidates for searching for sub-Alfvénic interactions, raising the question whether LHS~1610~b could be driving the flares on its host star. However, the available TESS photometry is insufficient to confirm or rule out any orbital phase-dependence of the flares. We show that the LHS 1610 system, as a nearby mid M star with a large, short-period companion, is a promising target to look for evidence of sub-Alfv\'enic interactions or auroral emission from the brown dwarf at radio wavelengths.
%\end{abstract}

% To this end, we show that LHS 1610 shares similar properties with other mid M dwarfs systems---such as Proxima Cen and YZ Ceti---that have recently discovered radio detections compatible with sub-Alfv\'enic interactions. 
%other mid M dwarfs with close-in companions with recently 
% With a flare rate of $0.28\pm 0.07$ flares/day, and a rotation period of $84 \pm 8$ days, LHS 1610 shares similar properties 
%joins a growing group of mid M stars with close-companions with high flare rates but long rotation periods, where both Both Proxima Cen and YZ Ceti have candidate claimed radio detections 
%These stars are promising candidates for searching for sub-Alfvénic interactions, raising the question whether LHS~1610~b could be driving the flares on its host star. However, the available TESS photometry is insufficient to confirm or rule out any orbital phase-dependence of the flares.
%We show that LHS 1610 joins a growing group of other mid M stars with close-in companions that have high flare rates and long stellar rotation periods, 
%We show that the available TESS photometry is insufficient to determine an orbital phase-dependence of the flares.
%additionally show that LHS 1610 has a high flare rate ($0.28\pm 0.07$ flares/day) for its long rotation period ($84 \pm 8$ days), 
%To this end, we show that LHS 1610 joins a growing group of other mid M stars that have high flare rates 
%Additionally, with a flare rate of $0.28\pm 0.07$ flares/day from TESS photometry, and a rotation period of $84 \pm 8$ days, LHS 1610 joins other mid M stars---including Proxima Centauri and YZ Ceti---as nearby mid M dwarfs with flare rates on the higher end for their long rotation periods. These stars are promising candidates for searching for sub-Alfvénic interactions, raising the question whether LHS~1610~b could be driving the flares on its host star. However, the available TESS photometry is insufficient to confirm or rule out any orbital phase-dependence of the flares. }
%\updated{We measure the true mass ($ 49.5_{-3.5}^{+4.3}$ $M_{\text{Jup}} $) and inclination ($ 114.5^\circ$ $_{-10.0}^{+7.4}$) of the nearby ($d=9.7$ pc) brown dwarf LHS~1610~b by combining discovery radial velocities (RVs) from TRES and new RVs from the Habitable-zone Planet Finder with the available Gaia astrometric two-body solution. We highlight a discrepancy between the measurement of the eccentricity from the Gaia two-body solution ($e=0.52 \pm 0.03$) and the RV only solution ($e=0.3702\pm0.0003$). Possible reasons for this discrepancy are discussed, and we support future investigations into the cause when the Gaia astrometric time series are made available in Gaia Data Release 4. With a flare rate of $0.28\pm 0.07$ flares/day from TESS photometry, and a rotation period of $84 \pm 8$ days, the M5 dwarf LHS 1610 joins other mid M stars---including Proxima Centauri and YZ Ceti---as nearby mid M dwarfs with flare rates on the higher end for their long rotation periods. These stars are promising candidates in the search for sub-Alfvénic interactions, raising the question whether LHS~1610~b could be driving the flares on its host star. The available TESS photometry is insufficient to determine an orbital phase-dependence of the flares. We show that the LHS 1610 system, as a nearby mid M star with a large, short-period ($10.6$ day) companion, is a promising target to look for evidence of sub-Alfv\'enic interactions or auroral emission from the brown dwarf at radio wavelengths.}
%\updated{We measure the true mass ($ 49.5_{-3.5}^{+4.3}$ $M_{\text{Jup}} $) and inclination ($ 114.5^\circ$ $_{-10.0}^{+7.4}$) of the nearby ($d=9.7$ pc) brown dwarf LHS~1610~b by combining discovery radial velocities (RVs) from TRES and new RVs from the Habitable-zone Planet Finder with the available Gaia astrometric two-body solution. We highlight a discrepancy between the measurement of the eccentricity from the Gaia two-body solution ($e=0.52 \pm 0.03$) and the RV only solution ($e=0.3702\pm0.0003$). Possible reasons for this discrepancy are discussed, and we support future investigations into the cause when the Gaia astrometric time series are made available in Gaia Data Release 4. With a flare rate of $0.28\pm 0.07$ flares/day from TESS photometry, and a rotation period of $84 \pm 8$ days, the M5 dwarf LHS 1610 joins other mid M stars---including Proxima Centauri and YZ Ceti---as nearby mid M dwarfs with flare rates on the higher end for their long rotation periods. These stars are promising candidates in the search for sub-Alfvénic interactions, raising the question whether LHS~1610~b could be driving the flares on its host star. The available TESS photometry is insufficient to determine an orbital phase-dependence of the flares. We show that the LHS 1610 system, as a nearby mid M star with a large, short-period ($10.6$ day) companion, is a promising target to look for evidence of sub-Alfv\'enic interactions or auroral emission from the brown dwarf at radio wavelengths.}
%\updated{We characterize the LHS 1610 system, a nearby ($d=9.7$ pc) M5 dwarf hosting a brown dwarf in a $10.6$ day, eccentric ($e \sim 0.37$) orbit. By combining discovery radial velocities (RVs) from TRES with new RVs from the Habitable-zone Planet Finder we derive an updated minimum companion mass of $44.38\pm0.67$ $M_{\text{Jup}}$. We combine the RVs with the available Gaia astrometric two-body solution and constrain an inclination of $i=114.5^\circ$ $_{-10.0}^{+7.4}$ and true mass of $m=49.5_{-3.5}^{+4.3}$ $M_{\text{Jup}}$, confirming the brown dwarf nature of the companion. We highlight a discrepancy between the measurement of the eccentricity from the Gaia two-body solution ($e=0.52 \pm 0.03$) and the RV only solution ($e=0.3702\pm0.0003$). We discuss possible reasons for this discrepancy, and support future investigations into the cause when the Gaia astrometric time series are made available in Gaia Data Release 4. Additionally, with a flare rate of $0.28\pm 0.07$ flares/day from TESS photometry, and a rotation period of $84 \pm 8$ days, LHS 1610 joins other mid M stars---including Proxima Centauri and YZ Ceti---as nearby mid M dwarfs with flare rates on the higher end for their long rotation periods. These stars are promising candidates for searching for sub-Alfvénic interactions, raising the question whether LHS~1610~b could be driving the flares on its host star. However, the available TESS photometry is insufficient to confirm or rule out any orbital phase-dependence of the flares. We show that the LHS 1610 system, as a nearby mid M star with a large, short-period companion, is a promising target to look for evidence of sub-Alfv\'enic interactions or auroral emission from the brown dwarf at radio wavelengths.}

% Without the actual astrometric data, it is impossible to isolate the cause of this discrepancy, and we urge that the  joint \updated{sampling will} need to be revisited when the individual Gaia astrometric time-series are released as part of Gaia DR4.
% \updated{If we assume the inclination estimate from the two-body solution is correct, pairing this with our minimum mass measurement, we would derive a true mass of $44.45\pm0.67$ $M_{\text{Jup}}$}. However, 
% Although \updated{the values for the time of periastron and $\omega$ are consistent} between the RV-only solution and the Gaia two-body solution, we see a discrepancy between the eccentricity \updated{and period} from the two-body solution of 
% To reflect this, for the joint \updated{sampling}, we placed a uniform prior on $\cos i$ from -1 to 0 (see Table \ref{tab:priors}).

%The off diagonal elements are the covariances between the corresponding parameters of the intersection. This means that for some off-diagonal index of parameters X and Y, then cov(X,Y) $= \rho_{\text{xy}} \sigma_{\text{x}} \sigma_{\text{y}}$, where $\rho_{\text{xy}}$ is the correlation factor between the parameters, and the $\sigma$'s are the standard deviations on each respective parameter. This means that we double up on the scale factor since we are increasing everything homogeneously, hence the broad multiplication by the square of the scaling factor.
